Targeted Extraction of Temporal Facts from Textual Resources for Improved Temporal Question Answering over Knowledge Bases

Knowledge Base Question Answering (KBQA) systems have the goal of answering complex natural language questions by reasoning over relevant facts retrieved from Knowledge Bases (KB). One of the major challenges faced by these systems is their inability to retrieve all relevant facts due to factors such as incomplete KB and entity/relation linking errors. In this paper, we address this particular challenge for systems handling a specific category of questions called temporal questions, where answer derivation involve reasoning over facts asserting point/intervals of time for various events. We propose a novel approach where a targeted temporal fact extraction technique is used to assist KBQA whenever it fails to retrieve temporal facts from the KB. We use $\lambda$-expressions of the questions to logically represent the component facts and the reasoning steps needed to derive the answer. This allows us to spot those facts that failed to get retrieved from the KB and generate textual queries to extract them from the textual resources in an open-domain question answering fashion. We evaluated our approach on a benchmark temporal question answering dataset considering Wikidata and Wikipedia respectively as the KB and textual resource. Experimental results show a significant $\sim$30\% relative improvement in answer accuracy, demonstrating the effectiveness of our approach.

==> tmp/intro.tex <==
\section{Introduction}
% introduction text
Complex Question Answering has been important both from an applicative point-of-view, as such questions naturally arise in real life, and from a scientific point-of-view, as they allow us to test the reasoning abilities of our models. It has caught the interest of researchers working in the space of NLP and reasoning lately \cite{vakulenko2019message, maheshwari2018learning, saxena-etal-2020-improving, fu2020survey, bhutani-etal-2020-answering, wu2021modeling}. Complex questions are those that require integrating facts over multiple pieces of disjoint information (also called “multi hop”). In this paper, we specifically deal with temporal questions. These questions require fetching time intervals of various events in the question and additionally require temporal reasoning to resolve the intervals to fetch the correct answer. For example, one such question is, “Who was the President of the United States during World War 2 ?”. In order to correctly answer this question, we require the time interval of World War 2, along with the Presidents of the United States with their time intervals. We then need to perform temporal reasoning to fetch the President whose interval overlaps with the interval of World War 2.

Knowledge Bases (KBs) have proven to be an ideal source to answer such questions that involve multi-hop reasoning \cite{bhutani-etal-2020-answering, vakulenko2019message, wu2021modeling}. Knowledge Graphs (KGs) or Knowledge Bases are multi-relational graphs consisting of millions of entities (nodes) and relations (edges). Some of the large-scale multi-relational KGs are DBPedia \cite{Lehmann2015}, Freebase \cite{Bollacker2008} and WikiData (cite). WikiData is the largest publicly available KB with over 94.7 million data items as of August 2021. It is also
fast evolving and the most up-to-date KB, hence we use WikiData for our experiments in this work. Traditional KBQA approaches to handle Complex Questions have used neural models \cite{maheshwari2018learning, vakulenko2019message, fu2020survey}, and neuro-symbolic approaches \cite{kapanipathi2021leveraging}

Conversely, corpus based question answering is a problem that has been studied in vast detail in the recent past \cite{zhang2020retrospective, zhang2019sgnet, saha-etal-2018-duorc}. This approach is well suited for simple one-hop questions that require very minimal reasoning. Reading comprehension tasks have a context provided along with the question, whereas open domain QA involving retrieval of relevant documents is a relatively complex problem given the amount of text that needs to be processed in order to find facts needed to answer. Open domain QA has seen considerable success in the past\cite{chen2017reading, wang2018evidence, wang2017r3}. However an Open domain approach to answer complex questions has its drawbacks. For example, it is relatively hard to get the exhaustive list of US presidents along with their interval from Wikipedia text alone. Not all the US presidents are mentioned in the text of the Wikipedia page, “President of the United States“. Many of the presidents are mentioned in tables and images from where extraction is relatively difficult. However, it is easier to get the list of US presidents from a KB which has structured data. This makes KB highly suitable for reasoning based multi-hop QA.

Although KBs are the most preferred source to solve multi hop QA as they have a structured way of storing information,  KBs have long proven to suffer from issues such as missing and incomplete facts \cite{jain2020temporal, lacroix2020tensor, garcíadurán2018learning}. Adding to these are the inevitable errors(cite emnlp paper) that arise in Entity \cite{wu-etal-2020-scalable} and Relational Linking \cite{Mihindukulasooriya_2020} that serve as crucial stages in the answering process. In this work, as we specifically deal with temporal questions, we observe that temporal facts are more commonly missing or incomplete in WikiData. In order to bridge these issues we propose a novel approach that performs a targeted temporal fact extraction from textual resources,  Wikipedia in our case. The proposed system attempts to answer temporal questions with the help of WikiData (KB) and identifies missing or incomplete facts within the KB, if any. It then performs a KB-guided textual look-up to extract these missing facts from text in order to answer the questions. 

\begin{table*}[th]
\centering
\begin{tabular}{|c|c|c|}
\hline
                      & \textbf{Single Hop}            & \textbf{Multi Hop}                                        \\ \hline
\textbf{Non Temporal} & Who directed Jurassic Park?    & What is the nationality of the director of Jurassic Park? \\ \hline
\textbf{Temporal}     & When was Abraham Lincoln born? & Who was the President of USA before Abraham Lincoln?      \\ \hline
\end{tabular}
\end{table*}


\noindent Our main contributions in this work are as follows:
\begin{itemize}
\item We propose a novel and highly interpretable neuro-symbolic approach that leverages text resources and performs a KB guided textual extraction to fetch what’s missing in KB. In essence, we bring out the best of both worlds to answer temporal questions (KB and Text). To the best of our knowledge, this is the first attempt to answer temporal questions from multiple knowledge sources (WikiData and Wikipedia).
\item The approach employed is closest to human intuitions used to answer such questions. Moreover, we propose a first of its kind Question Understanding module that leverages semantic parsing \cite{zhou2021amr} to decompose multi-hop questions into simpler sub-questions for easier interpretability and human-like temporal reasoning.
\item We propose a simple and a highly effective approach leveraging pre-trained neural models for fact extraction from text by using targeted text queries which are in turn generated from lambda expressions that capture the meaning of what we are looking for. Furthermore, we demonstrate the effectiveness of the fact extraction module even without domain-specific fine-tuning.
\item Our proposed strategy improves the SOTA substantially on the benchmark TempQA-WD dataset \cite{Jia2018} which is the widely used dataset consisting of Temporal Questions.


\end{itemize}



~

==> tmp/kb+text.tex <==
\subsection{Textual Extraction}
% description of the overall approach
This section describes the modular textual extraction approach that performs target temporal fact extraction from Wikipedia. Our approach to fetch facts is guided by the KB. More specifically, we look only for what's missing and prune down the search space effectively. Prior works of open domain text retrieval have used different techniques for passage retrieval. BM25 \cite{Robertson2009} is the first successful approach to retrieve documents through keyword matching by representing the question and passages as a high dimensional, sparse vector space. Off late, the dense retrieval mechanisms have shown considerable improvements over the BM25 or TF-IDF methods \cite{lee2019latent, karpukhin2020dense}.

Our proposed modular approach retrieves documents using a lexical matching approach. Documents are essentially Wikipedia pages. For the same we generate textual queries from lambda expressions. These queries express the auxiliary or main lambda in NL form. This is necessary as retrieval of documents, re-ranking and fact extraction require a query in textual form. We then re-rank the retrieved passages before using a pre-trained BERT model as reading comprehension task to answer the query based on the most relevant passages. The pipeline consists of the following modules, 1) Lambda To TextQuery, 2) Document Retrieval, 3) Top Relevant passages and Re-ranking,  4) Bert Based fact Extraction, 5) AMR Parse Tree for end date resolution
~

\subsubsection{Lambda To TextQuery:}
% what are we looking to extract from text based on what is missing in the KB
At every stage of the fact extraction process, we use queries generated from Lambda expressions that capture it’s meaning. For example, if we are looking for the missing auxiliary fact of the example stated above. The lambda expression that captures the auxiliary is lambda ri. release-01(r, “Ankahee”) interval(ri, r). We generate a query, “When did Ankahee release?”. It is clear that we always look for a temporal fact and hence, our fact extraction query would always start with “when”/”what year”. The next verb “release” comes from the predicate of Auxiliary lambda followed by the entity Ankahee. Another example would be to look for the tenure of Tim Pawlenty as the Minnesota Governor. The main lambda would have the form, “lambda a. have-org-role-91(a, governor, Minnesota). One of the many candidates obtained from KB would be Tim Pawlenty. The query generated would be of the form, “When was Tim Pawlenty  Governor of Minnesota?”. It can be understood that our query has to be temporal and would invariably follow the template: “When was/did [Entity] [Action] ?”. This query is used to retrieve documents, re-rank passages and finally to answer questions as a reading comprehension task.

~

\subsubsection{Document Retrieval: }
% description of retrieval
The document retriever happens at 2 stages. Firstly we collect the Wikipedia pages of all the entities mentioned in the complete question, regardless of the missing fact we are looking for(main or aux). For the above example, the 2 entities are the Governor of Minnesota and Ankahee. We use fuzzywuzzy \footnote{https://chairnerd.seatgeek.com/fuzzywuzzy-fuzzy-string-matching-in-python/} to perform fuzzy string match to the closest Wikipedia page that overlaps with the entity. For example, there is no Wikipedia page called “Ankahee” and this needs to be linked to, “Ankahee (2006 film)” which would have the highest fuzzy match score with Ankahee. The Wikipedia content is accessed using Wikipedia API (link). We extract the entities from the question using BLINK \cite{wu2019general}.

The next set of documents would be query specific. We use the MediaWiki API \footnote{https://www.mediawiki.org/wiki/Download} 
to search the documents related to the query generated from lambda expression. First, we send a query to get a list of related pages. Then the contents of the top 3 relevant pages are fetched. This fetches pages based on frequency of word occurrences and is useful because sometimes Wikipedia pages about multiple entities have information that may prove useful. For example, there exists a Wikipedia page, “Argentina–Spain relations”, whose contents will have answers to questions like, “When did Spain invade Argentina?”, which cannot be answered by documents from either Spain or Argentina’s individual wiki Page. Hence this second route of using query keywords generated from lambda expression to fetch pages with highest frequency overlap becomes crucial.
~

\subsubsection{Top Relevant passages and Re-ranking}
% description of how do we extract temporal facts

Now that we have extracted a collection of documents, the next step would be to look for the most relevant passages from the document collection. We use the Bi-encoder, Cross-Encoder based Siamese-BERT networks \cite{reimers2019sentencebert} to re-rank passages based on the query generated from lambda expression. Bi-Encoder picks out the top 50 relevant passages based on passage-query similarity and Cross-Encoder re-ranks the top passages. Both the neural models are trained for the specific task on the MS-MARCO dataset \cite{bajaj2018ms}. We use the pre-trained checkpoints of the model open-sourced by sentence-transformers \footnote{https://www.sbert.net/}

~

\subsubsection{Bert Based fact Extraction}
% how do we reform lambda expression using facts found from text

We treat the fact extraction as a reading comprehension task using the top 3 relevant passages that is ranked by the Cross Encoder as context and the question generated using the Lambda To Text Query as explained earlier. We leverage BERT checkpoints from HuggingFace \footnote{https://huggingface.co/} pre-trained on the SQUAD data set \cite{rajpurkar-etal-2016-squad}. We also demonstrate that this QA model trained on SQUAD itself gives significant increase in performance without any task-specific(Temporal QA) pre-training that is limited by the unavailability of large training data.
~

\subsubsection{AMR Parse Tree for end date resolution}
% how do we derive answer
The pre-trained BERT QA model will fetch only one answer from the context, and it would be the start date of a particular event ( although end date is possible in a few cases ), we use AMR semantic parse tree to fetch the end date. We perform semantic parsing of the sentences in the context and traverse the edges of the AMR parse tree and look for the BERT extracted date node, we then look for another date entity that is present as a sibling node to this date node. These two date intervals will represent the entire tenure of an event. However, it is observed that in a few cases that both the end and start dates are not simultaneously mentioned within the top 3 relevant passages. Hence, our system does not fetch a bounded interval in such cases. This is one of the major drawbacks of such a text extraction system where a single document may contain only partial temporal information of an event. The figure explains this approach in detail.
~



==> tmp/kbqa.tex <==
\subsection{KBQA}
% a brief description of KBQA
In this section we give a brief description of the Neuro Symbolic KBQA appraoch proposed in  (cite emnlp paper). We refer the readers to the paper for more details. Our work builds on top of this KBQA pipeline.

The system leverages AMR semantic parsing \cite{zhou2021amr} to convert the question into a logical representation that captures the underlying semantics. We use the same algorithm proposed in (cite emlp paper) to convert the AMR tree into a logical expression. The logical representation uses the formalism of Typed Lambda Calculus presented in \cite{zettlemoyer2012learning}. The system then uses Entity Linking and Relational Linking module as proposed in \cite{wu-etal-2020-scalable} and \cite{Mihindukulasooriya_2020} respectively. This is followed by conversion into a KB specific Lambda expression and a subsequent SPARQL query generation which is then used to fetch answers from WikiData. As our work builds on top of this system and extensively uses the intermediate logical representation (Lambda logic) to decompose questions, we describe the Lambda Calculus in brief in the coming sections.
~

\subsubsection{Lambda Expression}


This section briefly introduces Lambda expressions for the question. Show some examples as well

Question: When was Donald Trump born?

Logical Form: \textit{λt. born(b,“Donald Trump") ∧
interval(t, b)}



~

\subsubsection{Question Decomposition:}
% briefly about question understanding, lambda expression
This section describes a crucial stage of the proposed approach that enables identification of missing facts in KB. Question decomposition is crucial to solve multi-hop questions as they require integrating multiple pieces of information. In most cases, temporal questions are comprised of 2 sub-questions and absence of answer to even one of the two, means we do not have enough facts to derive the final answer. Hence question decomposition helps us in "probing" what's missing in KB, which is described in the following section.

TEQUILA \cite{Jia2018} proposes to decompose questions at a sentence level in it's natural language form, which gives rise to erroneous results if the question doesn't follow a specific template, whereas we propose to decompose the logical representation of the question taking into account it's semantics. Concretely, we term the sub-question that often contains the unknown as "main", and the supplementary sub-question that is needed for the reasoning step as "auxiliary". For example, the question, " \textit{"Who was the President of the United States  during World War 2"} has a main sub-question as, \textit{"Who was the President of the United States ?"} and auxiliary sub-question as, \textit{"When did World War 2 happen?"}. As described earlier, a naive sentence level decomposition using predefined templates do not work in cases where questions are phrased non-trivially. Acknowledging these shortcomings, our approach decomposes the Lambda Expression of the question itself into main lambda and auxiliary lambda that capture the semantics of the main and auxiliary sub-questions respectively. Below is an example:



Question: Who was the President of the United States during World War 2?

% Question Lambda: \textit{λa. have-org-role-91(h, a, "United States", "president") ^  interval(hi, h) ^ interval(ri, "World War 2") ^  overlap(hi, ri) }

Main Lambda: \textit{λa. have-org-role-91(h, a, "United States", "president")}

Auxiliary Lambda: \textit{λri. interval(ri, "World War 2")}

Essentially, when the main lambda is passed to the KBQA system, we get the names of all US presidents from WikiData. This is because the unknown variable "a" in the main lambda is satisfied by entities that are US presidents. When the Auxiliary lambda is passed to the KBQA system we get the interval of World War 2 from WikiData. The process used to methodologically decompose complex lambdas into main and auxiliary lambda is explained in Algorithm 1. ( Make algo table)

~

\subsubsection{Probing what's missing in KB}
The first step to improvise any system is to understand why and how it fails. That is, we attempt to answer the given question using only KB as the information source, and if it fails we identify the missing fact that is the cause of failure. This missing fact is then fetched from an alternate information source, i.e., text. Concretely, we go into text and perform a guided fact extraction to get the facts missing in KB. These facts are then used along with the KB gathered facts to answer via temporal reasoning. In order to know what's needed/missing we need to prob the only KB system to see why it fails to give an answer. The failure of the only KB pipeline could possibly happen at two levels:
\begin{itemize}
\item  \textbf{Aux Failure:} Auxiliary interval or entity missing in KB. For example, the interval of World War 2 could be possibly missing in KB due to which the pipeline fails to reason and come up with a decisive answer
\item  \textbf{Main Failure:} Main Candidate missing or corresponding interval incomplete in KB. By this we mean one of the potential answer candidates could be missing or incomplete within the KB. For example, Franklin D. Roosevelt's (US president during World War 2) tenure interval could possibly be missing within the KB, due to which the only KB pipeline fails to give out any answer.

\end{itemize}

This work attempts to  specifically address this issue of missing/incomplete facts in KB by fetching the missing intervals through textual extraction, specifically from Wikipedia pages of the missing entities. (Put a figure or algorithm table that explains this if-else condition of what to do )



% briefly about linking
~

\subsubsection{Aux Failure:}
(A clear image running through this example)
As mentioned earlier, this occurs because of the missing auxiliary fact within KB. For example, as explained in figure the only KB pipeline fails to answer the  question "Who was the Governor of Minnesota when Ankahee released?". On probing, the reason for the failure was the erroneous entity linking of the entity "Ankahee". In order to resolve it, we fetch the release date of the film Ankahee from the Wikipedia page of the entity. This is followed by reforming the lambda expression by hard-coding the correct date. The predictes release-01(r, "Ankahee") interval(ri, r) gets replaced by interval(ri, date("dd-mm-2006"). The reformed lambda expression is now used to fetch the final answer from KB. This time the KBQA system doesn't need to look for release date of Ankahee from the KB as it is explicitly mentioned in the lambda expression. It has to perform "overlap" temporal reasoning operation with tenures of all Minnesota Governors and the date 2006 . The details of how we extract the year "2006" from text is explained in the coming sections (Textual Extraction section).

\textbf{Question}: Who was the Governor of Minnesota when Ankahee was released?

\textbf{Original Lambda}: lambda a. have-org-role-91(h, a, "Minnesota", governor) interval(hi, h) \textbf{release-01(r, "Ankahee") interval(ri, r)} overlap(hi, ri)

\textbf{Reformed Lambda}: lambda a. have-org-role-91(h, a, "Minnesota", governor) interval(hi, h) \textbf{interval(ri, date("dd-mm-2006")} overlap(hi, ri)
% briefly about KB facts extraction and reasoning

If the reformed lambda fails to fetch answers from KB, it is an indicator that there is incomplete information with respect to the main candidates. This leads us to the next stage. One important point to note here is that even if the reformed lambda fails to fetch answer from KB, fetching and storing the correct auxiliary interval from text helps in later stages of the pipeline.
~

\subsubsection{Main Failure}
This failure could be detected if either of the following occur: 1) The Auxiliary fact is present in KB, but still our KBQA system doesn't fetch an answer. 2) The missing Auxiliary fact has been attended to by fetching the auxiliary date, but still the reformed lambda expression doesn't fetch valid answer. In these two cases the reason of failure has to be one or many of the main candidates. It could be a problem with linking entities to their KB counterparts or once again, missing temporal information. 

We propose to resolve this issue by fetching all the answer candidates (For example, list of all US Presidents, or list of all Minnesota Governors). This could be simply done by using the main lambda expression to fetch main candidates from KB. These candidates are all potential answers to the question, as they satisfy main lambda but are yet to be constrained by the auxiliary lambda. For each of these candidates, we subsequently fetch the time intervals of their tenure through text extraction. It is important to note that fetching these intervals from KB would be redundant, as the reason for the main failure itself is the missing temporal fact. The details of this text extraction is explained in detail in the coming section. Once we have the time interval/points in time for each main candidate, and the auxiliary time interval obtained either through KB, if not then text, we move on to the final stage of temporal reasoning to fetch answers.


\subsubsection{Temporal Reasoning}

Following the works of TEQUILA \cite{Jia2018}, we have three broad temporal categories to classify the questions. They are "before", "after" and "overlap". Although, the categorization could happen at the sentence level by detecting trigger words in question itself like previous works, we perform this categorization through the logical representation ( lambda expression ) of the question to avoid pre-defining templates and signal words that do not guarantee a robust system. The table shows examples of all the three categories. This temporal reasoning step is performed explicitly only when there is main failure. As in this case we explicitly collect temporal facts about each of the candidate and then resolve it with auxiliary interval to get the answer. In case of auxiliary failure, this step is carried out internally by the KBQA engine while fetching answers from KB using reformed lambda.

\textbf{Overlap}: This reasoning operation looks for all main candidates whose start date<= auxiliary interval<= end date.

\textbf{Before}: This operation is satisfied by argmax(i) st. (end date(i) <= auxiliary date.

\textbf{After} This operation is satisfied by argmin(i) st. ( start date (i) >= auxiliary date.

\begin{table*}[th]
\begin{tabular}{|l|l|l|}
\hline
\textbf{Category} & \multicolumn{1}{c|}{\textbf{Question}}                   & \textbf{Lambda Expression} \\ \hline
Overlap                    & Who was the Governor of Minnesota when Ankahee released? &                            \\ \hline
Before                     & Who was the London Mayor before Boris Johnson?           &                            \\ \hline
After                      & What team did Allen Iverson play for after the 76ers?    &                            \\ \hline
\end{tabular}
\end{table*}

